FLAIR: Feeding via Long-horizon AcquIsition of Realistic dishes

Robot-assisted feeding has the potential to improve the quality of life for individuals with mobility limitations who are unable to feed themselves independently. However, there exists a large gap between the homogeneous, curated plates existing feeding systems can handle, and truly in-the-wild meals. Feeding realistic plates is immensely challenging due to the sheer range of food items that a robot may encounter, each requiring specialized manipulation strategies which must be sequenced over a long horizon to feed an entire meal. An assistive feeding system should not only be able to sequence different strategies efficiently in order to feed an entire meal, but also be mindful of user preferences given the personalized nature of the task. We address this with FLAIR, a system for long-horizon feeding which leverages the commonsense and few-shot reasoning capabilities of foundation models, along with a library of parameterized skills, to plan and execute user-preferred and efficient bite sequences. In real-world evaluations across 6 realistic plates, we find that FLAIR can effectively tap into a varied library of skills for efficient food pickup, while adhering to the diverse preferences of 42 participants without mobility limitations as evaluated in a user study. We demonstrate the seamless integration of FLAIR with existing bite transfer methods [19, 28], and deploy it across 2 institutions and 3 robots, illustrating its adaptability. Finally, we illustrate the real-world efficacy of our system by successfully feeding a care recipient with severe mobility limitations. Supplementary materials and videos can be found at: https://emprise.cs.cornell.edu/flair .

==> figures/plate_runs.tex <==
\begin{figure}[ht!]
 \centering
  \includegraphics[width=0.5\textwidth]{figures/src/plate_runs.png} % Adjust the width as necessary
  \caption{Plates used for evaluation, covering a wide range of food items.}
  \label{fig:plate_runs}
\end{figure}

==> figures/teaser.tex <==
\begin{figure}[ht!]
 \centering
  \includegraphics[width=0.5\textwidth]{figures/src/Frame 3.png} % Adjust the width as necessary
  \vspace{-1cm}
  \caption{We propose a novel method that leverages Foundation Models for long-term task planning in bite acquisition. Our method enables human-like feeding of complete meals containing various food items, by balancing between user preferences and efficient plate clearance. }
  \vspace{-0.5cm}
  \label{fig:teaser}
\end{figure}

==> inputs/introduction.tex <==
\label{sec:intro}

\section{Introduction}

% Para 1: Motivation
Eating is vital to everyday life, yet millions worldwide struggle with it due to mobility limitations, age, or health conditions~\cite{taylor2018americans}. These individuals often rely on caregivers for meal assistance, impacting the individual's independence, daily routines, and the social experience of dining~\cite{jacobsson2000eatingprocess, nanavati2023design, shune2020experience}. Moreover, feeding is one of the most time-consuming Activities of Daily Living for caregivers~\cite{chio2006caregiver}. Robot-assisted feeding holds promise for improving the quality of life for those requiring assistance~\cite{brose2010role}, and reducing the burden on caregivers. 

Robot-assisted feeding consists of two stages: bite acquisition and bite transfer~\cite{madan2022sparcs}. While various prior works tackle bite transfer~\cite{belkhale2022balancing, shaikewitz2022mouth, jenamani2024bitetransfer}, which entails moving a food item to a care recipient's mouth, they typically assume that the food item of choice has already been picked up from the plate. However, this process of \emph{bite acquisition} is a challenging interplay of nuanced low-level manipulation to pick up foods of drastically different properties, along with high-level decision making over the sequence of bites to feed over a long horizon. 

Due to the wide range of visual appearances and physical textures food encompasses, different food groups necessitate distinct manipulation strategies such as skewering, scooping, or cutting. Several prior works have focused on developing individual skills that address each of these strategies in isolation, such as training policies from self-curated food datasets to skewer firm foods~\cite{feng2019robot, gordon2023towards, sundaresan2022learning}, scoop soft foods~\cite{grannen2022learning, tai2023scone}, rearrange and twirl noodles~\cite{sundaresan2023learning}, or cut non bite-sized items~\cite{zhang2019leveraging}. While specialization in handling different food items is vital, feeding a complete meal comprising various food items to a care recipient in a real-world setting demands unifying these approaches under a complete library of acquisition skills, effectively sequencing these skills over a long-horizon, and seamlessly integrating acquisition with transfer. Despite significant advances in these areas individually, developing a system that cohesively brings all these elements together remains an open challenge.

% Discuss bite sequencing as utensil -> efficiency -> preference. Key Idea.
When building a repertoire of parameterized skills for acquisition, an important consideration is how to \emph{sequence} available skills over a long-horizon to feed plates in their entirety. Beyond practical considerations such as associating the appropriate acquisition skill with a perceived food item (i.e. skewering for carrots, scooping for mashed potatoes), feeding is a highly personalized experience. For example, consider a scenario where a robot is tasked with feeding a plate of spaghetti with meatballs on top to a user who prefers to eat all the spaghetti initially. The robot must be able to infer the need to push one or several meatballs aside in order to twirl a pile of spaghetti beneath. Another important consideration, however, is the pace of the meal. It may be painstakingly slow to move aside each meatball just to get to a bite of spaghetti. Skewering a meatball might be a much quicker option for a more ambivalent user. The key idea for effectively sequencing bites over a long-horizon is to respect a user's \emph{preferred} ordering while also considering \emph{efficiency}.


% When building a repertoire of parameterized skills for acquisition, an important consideration is how to \emph{sequence} available skills over a long-horizon to feed plates in their entirety. Beyond practical considerations such as associating the appropriate acquisition skill with a perceived food item (i.e. skewering for carrots, scooping for mashed potatoes), effective skill sequencing requires taking into consideration the sequensemanipulation actions required for food pickup and user preferences. For example, 

% feeding is a highly personalized experience. For example, consider a scenario where a robot is tasked with feeding a plate of spaghetti with meatballs on top to a user who prefers to eat all the spaghetti initially. The robot must be able to infer the need to push one or several meatballs aside in order to twirl a pile of spaghetti beneath. Another important consideration, however, is the pace of the meal. It may be painstakingly slow to move aside each meatball just to get to a bite of spaghetti. Skewering a meatball might be a much quicker option for a more ambivalent user. The key idea for effectively sequencing bites over a long-horizon is to respect a user's \emph{preferred} ordering without compromising on \emph{efficiency}.

% FLAVORS
In this work, we introduce a robot-assisted feeding system capable of feeding a complete meal comprising various food items to a care recipient in a real-world setting. 
% Line on foundation models here. 
Given visual observations of a plate, our approach first employs the zero-shot detection capabilities of Vision-Language Models (VLMs) to detect food items on the plate. Next, we associate per-item semantic labels with the appropriate acquisition strategies. Along with an optionally provided user preference in natural language, we next determine the pickup efficiency per-item by inferring the sequence of skills which would result in acquisition. Provided both, we generate bite sequences leveraging Large Language Models (LLMs). The few-shot summarization and common-sense reasoning capabilities of these models allow for interpreting user preferences, efficiency scores, and extrapolating sequences of bites that cater to both. 
% Finally, we carry out these sequences for long-horizon feeding in an MPC-style loop, via a library of skills comprising rearrangement, acquisition, and in-mouth-bite transfer.

We validate our system for long-horizon food pickup across 8 diverse plates ranging from in-the-wild dishes from DoorDash and prepared grocery store meals to homemade meals. In a user study across YY individuals, we use this system to demonstrate the necessity of balancing between both user preferences and efficiency for feeding complete meals, as compared to an efficiency-only or preference-only approach. Finally, we demonstrate the real-world effectiveness of our system by feeding a care-recipient with Multiple Sclerosis two meals -- an entree plate of spaghetti and meatballs, and a dessert plate of brownie bites, banana and chocolate sauce. (Conclude with findings from Kathleen.) 

At a glance, our contributions include: 
\begin{itemize}
    \item A robot-assisted feeding system with 7 specialized skills that can feed complete meals by leveraging foundation models for long-horizon bite sequencing  
    \item Comprehensive evaluations across 8 diverse plates evaluated by XX individuals, validating the effectiveness of considering both preferences and efficiency for feeding
    \item Demonstration of the real-world efficacy of our system for feeding a care recipient with mobility limitations
\end{itemize}

==> inputs/old_introduction.tex <==
\label{sec:intro}

\section{Introduction}
% Eating meals is such a fundamental aspect of everyday life, that we often overlook its importance and challenges. The process of eating a meal is an incredibly nuanced feat of human manipulation and decision-making. Humans effortlessly perform precise low-level movements like orienting and positioning a fork properly to pick up a food item, while still reasoning at a high-level about the plate, such as deciding which bite to take next. Beyond these observations, the act of eating itself is often taken for granted. In reality, millions of individuals worldwide are unable to feed themselves independently due to mobility impairments, or age and health-related afflictions. Many of these individuals require caregiver assistance during meals, which can have an enormous impact on one’s sense of independence, routine, and the social aspect of dining. As a result, there is a huge potential for robots to provide mealtime assistance with the hope of reducing caregiver reliance and improving the quality of life of care recipients. 

% However, realizing a truly capable assistive feeding robot requires tackling the problem of diversity in a two-fold sense. First, there is an overwhelming diversity of dishes available that a feeding system must be equipped to handle. Secondly, every person differs in how they like to be fed. While some may have strong preferences over flavor combinations or bite orderings, others may not care to give explicit directions. The robot should still feed in a reasonable and efficient manner in all cases. For example, imagine a scenario where a robot is tasked with feeding a plate of spaghetti with meatballs on top to a user who prefers spaghetti. The robot needs to decide whether to push all the meatballs aside to get to the spaghetti, or to just pick up and feed a meatball first, which might be quicker. Alternatively, imagine feeding a plate of carrots, ranch, apples, and caramel. In the absence of explicit preferences from the user, the robot should be able to tell that carrots go with ranch, apples go with caramel, and that carrots and apples should be skewered while the sauces should be dipped. These scenarios challenge the robot to make sense of the visual plate in terms of what actions pair with which foods, and what sequence of bites would be most preferable and efficient.

% Several prior works in robot-assisted feeding focus on developing vision-parameterized skills for food pickup (i.e. skewering, or scooping), using segmentation or pose-estimation networks trained on hundreds to thousands of manually labeled food images or even demonstration trajectories. Even at this scale of supervision, resulting policies often do not generalize to out-of-distribution plates. Moreover, several of these works focus on a single or small set of specialized skills, like skewering or scooping in isolation, ultimately limiting the kinds of plates that can be fed. The prior systems that have attempted to sequence multiple available strategies tend to focus on specific but complex food groups like noodles, which benefit from proxy strategies like grouping noodles into piles, before pickup actions like twirling. Still, these approaches are too narrowly scoped to generalize to foods requiring other skills, and are largely concerned with efficient plate clearance without taking into account user-specific preferences over bite orderings. Our key insight is that we can leverage the few-shot reasoning capabilities of visual-language foundation models to infer truly general state-action representations for food items on a plate, while extrapolating general rules for efficient and personalized bite sequencing. This allows for a generalizable, zero-shot approach that handles diverse plates and preferences at scale.

% In this work, we present <method name>, a system for efficient and preference-informed long-horizon plate clearances. Given visual observations of a plate, our approach first employs the zero-shot detection capabilities of VLMs to estimate the visual state of food items on the plate and. Next, we use VLM summarization to associate detected food items and their semantic labels with appropriate skills from a library of available vision-parameterized skills, along with an estimate of the overall efficiency of picking up each food type. Finally, given an optional user-provided language description over their preferred ordering of bites, we defer to LLMs to plan preference and efficiency-informed sequences of bites, and execute the corresponding skills to achieve plate clearance.  
% Experimentally, we validate our approach across 8 diverse plates, requiring a range of pickup strategies, subject to varied preferences solicited across XX individuals. As compared to an efficiency-only or preference-only informed approach, we find that <method name> promotes the most natural and preferred bite sequences in a user study across YY individuals. 

% At a glance, our contributions include: 
% \begin{itemize}
%     \item A zero-shot system for preference-informed and efficient plate clearance with ZZ specialized skills, requiring no training
%     \item Comprehensive evaluations across 8 plates comprising home-cooked meals, prepared grocery store meals, and dishes ordered on DoorDash evaluated by YY individuals
%     \item A demonstration of our complete end-to-end system along with real bite transfer to a care recipient with mobility impairmnets
% \end{itemize}

% Para 1: Motivation
Eating is vital to everyday life, yet millions worldwide struggle with it due to mobility limitations, age, or health conditions \cite{taylor2018americans}. These individuals often rely on caregivers for meal assistance, impacting the individual's independence, daily routines, and the social experience of dining \cite{jacobsson2000eatingprocess, nanavati2023design, shune2020experience}. Moreover, feeding is one of the most time-consuming daily activities for caregivers \cite{chio2006caregiver}. Robot-assisted feeding holds promise for improving the quality of life for those requiring assistance \cite{brose2010role}, and reducing the burden on caregivers. 

Feeding consists of two key stages, namely bite acquisition, and bite transfer. A number of prior works have studied the challenges of \emph{bite transfer}, or bringing a bite of food to a user's mouth safely and comfortably, but critically assume that the food item of choice has already been picked up by the utensil. In reality, this process of \emph{bite acquisition} is one of the most nontrivial aspects of feeding itself. Bite acquisition is a challenging interplay of nuanced low-level manipulation to pick up foods of drastically different properties, along with high-level decision making over the sequence of bites to feed over a long horizon.

% Feeding involves two key stages: bite acquisition and bite transfer. Bite acquisition is the process of picking up a bite from the plate, whereas bite transfer pertains to safely and comfortably bringing the bite to the user's mouth. Although numerous studies have explored the complexities of bite transfer, there has been no prior research on feeding a complete meal that includes a variety of food items from a plate. This task presents a challenging interplay of nuanced low-level manipulation to pick up foods of drastically different properties, along with high-level decision making over the sequence of bites to feed over a long horizon.
% However, feeding a complete meal is a challenging interplay of nuanced food pickup strategies and long-horizon decision-making over the sequence of bites to feed.

% Para 2: Feeding is challenging and involves delicate balance. Present the challenges, our contributions and our key insight. 
Due to the wide range of visual appearances and physical textures food encompasses, different food groups necessitate distinct manipulation strategies such as skewering, scooping, or cutting. Several prior works have focused on developing individual skills that address each of these strategies in isolation, such as training policies from self-curated food datasets to skewer firm foods~\cite{feng2019robot, gordon2023towards, sundaresan2022learning}, scoop soft foods~\cite{grannen2022learning}, rearrange and twirl noodles~\cite{sundaresan2023learning}, or cut non bite-sized items~\cite{zhang2019leveraging}. While this degree of specialization is crucial for handling different food items appropriately, an assistive feeding system should unify each of these approaches under a complete library of acquisition skills, be able to sequence skills drawn from this library over a long-horizon, and seamlessly integrate acquisition with transfer for effective feeding. Prior work has made great strides towards these individually, but has yet to present a single system that is feature-complete.

When building a repertoire of parameterized skills for acquisition, an important consideration is how to \emph{sequence} available skills over a long-horizon to feed plates in their entirety. Beyond practical considerations such as associating the appropriate acquisition skill with a perceived food item (i.e. skewering for carrots, scooping for mashed potatoes), feeding is a highly personalized experience. For example, consider a scenario where a robot is tasked with feeding a plate of spaghetti with meatballs on top to a user who prefers to eat all the spaghetti initially. The robot must be able to infer the need to push one or several meatballs aside in order to twirl a pile of spaghetti beneath. Another important consideration, however, is the pace of the meal. It may be painstakingly slow to move aside each meatball just to get to a bite of spaghetti. Skewering a meatball might be a much quicker option for a more ambivalent user. The key idea for effectively sequencing bites over a long-horizon is to respect a user's \emph{preferred} ordering without compromising on \emph{efficiency}.

% achievable through harnessing the few-shot learning capabilities of foundation visual-language models.
% 


% Our key insight is that by framing feeding a complete meal as a bite sequencing problem that considers \emph{preference} and \emph{efficiency}, we can leverage the few-shot reasoning capabilities of visual-language foundation models to plan and execute personalized and efficient sequences of bites.

% Our key insight is that feeding a complete meal requires careful consideration of both \emph{preference} and \emph{efficiency} for planning sequences of bites, which is well suited to the few-shot reasoning capabilities of visual-language foundation models.

% Our key insight is  and we can leverage the few-shot reasoning capabilities of visual-language foundation models, along with a library of skills, to plan and execute bite sequences that address both.

% Our key insight is the necessity of harmonizing user preferences with efficiency in bite sequencing for robotic-assisted feeding, a balance achievable through harnessing the few-shot learning capabilities of foundation visual-language models.

% Prior works use perception modules trained on self-curated food datasets with limited generalization, and focus on a subset of the listed manipulation skills in isolation, developing specialized skills for picking up a standalone food item on a plate for a single bite.
% and then pickup the now exposed spaghetti balancing bite variety. Alternatively, imagine feeding a plate of carrots, ranch, apples, and caramel. In the absence of explicit preferences from the user, the robot should be able to tell that carrots go with ranch, apples go with caramel, and that carrots and apples should be skewered while the sauces should be dipped. 

% Report prior work here.

In this work, we introduce a robot-assisted feeding system that leverages a diverse library of food manipulation skills for user-preferred and efficient feeding. Given visual observations of a plate, our approach first employs the zero-shot detection capabilities of Vision-Language Models (VLMs) to detect food items on the plate. Next, we associate per-item semantic labels with the appropriate acquisition strategies. Along with an optionally provided user preference in natural language, we next determine the pickup efficiency per-item by inferring the sequence of skills which would result in acquisition. Provided both, we generate bite sequences leveraging Large Language Models (LLMs). The few-shot summarization and common-sense reasoning capabilities of these models allow for interpreting user preferences, efficiency scores, and extrapolating sequences of bites that cater to both. Finally, we carry out these sequences for long-horizon feeding in an MPC-style loop, via a library of skills comprising rearrangement, acquisition, and in-mouth-bite transfer.

We validate our system for long-horizon food pickup across 8 diverse plates ranging from in-the-wild dishes from DoorDash and prepared grocery store meals to homemade meals. In a user study across YY individuals, we use this system to demonstrate the necessity of balancing between both user preferences and efficiency for feeding complete meals, as compared to an efficiency-only or preference-only approach. Finally, we demonstrate the real-world effectiveness of our system by feeding a care-recipient with Multiple Sclerosis two meals -- an entree plate of spaghetti and meatballs, and a dessert plate of brownie bites, banana and chocolate sauce. (Conclude with findings from Kathleen.) 

At a glance, our contributions include: 
\begin{itemize}
    \item A robot-assisted feeding system with 7 specialized skills that can feed complete meals by leveraging foundation models for long-horizon bite sequencing  
    \item Comprehensive evaluations across 8 diverse plates evaluated by XX individuals, validating the effectiveness of considering both preferences and efficiency for feeding
    \item Demonstration of the real-world efficacy of our system for feeding a care recipient with mobility limitations
\end{itemize}

==> inputs/old_method.tex <==
\section{FLAIR: \underline{F}eeding via \underline{L}ong-horizon \underline{A}cquis\underline{i}tion of 
\underline{R}ealistic dishes}
In this section, we present \flair, a system for feeding complete meals which combines existing foundation models in a novel way towards personalized and efficient bite sequencing. We first give an overview of our custom system hardware, then outline our approach to long-horizon bite acquisition, and finally discuss integration of our method with existing bite transfer frameworks~\cite{gallenberger2019transfer, jenamani2024bitetransfer} for feeding of in-the-wild dishes. 

\begin{figure}
    \centering
\includegraphics[width=0.5\textwidth]{figures/rebuttal_figures/3embodiments_hardware.png}
    % \includegraphics[width=0.5\textwidth]{figures/hardware_utensil_full.png}
    \caption{We implement our skill library using a custom feeding utensil (adapted from~\cite{shaikewitz2022mouth}) having two degrees of freedom for easy twirling and scooping at the end effector. We deploy the full feeding stack on three robots and two institutions: the 7DoF Franka Emika Panda (top) and 7DoF Kinova Gen 3 (middle) at Stanford University, and the 6DoF Kinova Gen 3 (bottom) at Cornell University.} 
    \label{fig:hardware_setup}
    \vspace{-15pt}
\end{figure}


\subsection{Hardware System}
We tackle a wide range of food categories in this work such as fruits, vegetables, noodles, meat, soft foods, dipping sauces, and non-bite-sized items that require cutting. Many of these foods require specialized, dynamic manipulation strategies that typical 6 or 7-DoF robots struggle with due to their limited workspace. We thus implement \flair~on Kinova and Franka robot arms equipped with a motorized feeding utensil mounted at the end-effector, adapting the design from~\cite{shaikewitz2022mouth}. The utensil contains a fork attachment and has two degrees of freedom corresponding to the orientation of the fork tines and the tilt angle. This allows for directly controlling the utensil to perform dynamic movements like twirling and scooping, while the robot handles moving between waypoints in the workspace via Cartesian position control. We also use a wrist-mounted RGB-D Realsense camera with a known end-effector to camera transformation. This enables perceiving plates of food and localizing food items in the 3D workspace. We note that the same hardware was replicated on two different Kinova arms and one Franka Emika Panda, each with their separate fork attachment and sensors across two different institutions (detailed in Appendix), demonstrating the reproducibilty of our method and hardware (\added{\cref{fig:hardware_setup}}).

\subsection{Long-Horizon Bite Acquisition Framework}
\label{sec:bite_acq}
With access to a hardware platform that supports dexterous food manipulation strategies, our goal is to plan and execute long-horizon bite sequences that cater to a user's preference while efficiently feeding a meal.

\smallskip
\noindent \textbf{Problem Formulation.}
\label{sec:ps}
 We assume access to an RGB-D plate image observation $o_t \in \mathcal{O} = \mathbb{R}_{+}^{W \times H \times 4}$ of width $W$ and height $H$, and an optional natural language instruction $\ell_{pref}$ from the user, representing their preferred feeding strategy at a high-level (i.e., $\ell_{pref}$ = ``Feed me alternating bites of X and Y'' or ``Only feed me X''). X and Y can denote an arbitrary food item semantic label (i.e. ``spaghetti'', ``strawberry'', ``caramel'') or category (i.e. ``noodles'', ``fruit'', ``sauce''). 

We further assume access to a library $\mathcal{L} = \{\phi^1, \hdots, \phi^N\}$ of $N$ skills that the robot can use to manipulate food items. Each skill $\phi^i(p)$ represents a parameterized manipulation primitive that takes in parameters $p$ and outputs low-level motor commands. We represent a low-level action at time $t$ by $a_t = (x,y,z,\beta,\gamma)$, where $(x,y,z)$ denotes the position of the feeding utensil tip and $\beta$ and $\gamma$ denote pitch and roll, respectively. Thus, the output of any skill is a sequence of $T$ actions $\{a_t, a_{t +1}, \hdots, a_{t + T}\}$ that the robot takes to execute the particular strategy. For instance, a skewering skill may take the position and orientation of a desired food item as input, and output a trajectory that skewers the item of choice. Our goal is to plan and execute a sequence of parameterized skills $\{\phi_1(p_1), \phi_2( p_2), \hdots, \phi_H(p_H)\}$ which results in efficient and user-preferred bite acquisition, where $H$ is the total number of skills to execute to complete feeding a plate and $p_h$ refers to the parameters of skill $\phi_h \in \mathcal{L}$.

\begin{figure*}
    \centering
    \makebox[\textwidth][c]{%
    \includegraphics[width=1\textwidth]{figures/skills.png}
    }
    \caption{Our skill library consists of 7 parameterized manipulation skills: 4 acquisition (skewer, twirl, scoop, dip) and 3 pre-acquisition (group, push, cut).}
    \label{fig:front}
    \vspace{-15pt}
\end{figure*}


\smallskip
\noindent \textbf{State Representations for Food.}
Our approach addresses the main challenges in long-horizon bite acquisition—parameterizing low-level skills and sequencing them—by integrating state-of-the-art visual-language models. We use visual state estimates and semantic features of food items to guide skill parameterization and sequencing.

For a given plate observation $o_t$ at time t, we first query GPT-4V~\cite{achiam2023gpt} in a few-shot manner to recognize which food items are present. We prompt the model with 5 in-context examples of plate images and their corresponding ground truth food item semantic labels, and ask the model to complete the prompt for the test image $o_t$. GPT-4V outputs a list of semantic labels $l_t$ that are present, (i.e., $l_t = \texttt{[`fettuccine', 'chicken', `broccoli']}$) along with their corresponding categories $c_t$ (i.e., $c_t = [\texttt{`noodles'}, \texttt{`meat/seafood'}, \texttt{`vegetable'}, \texttt{`cuttable'}]$). These categories are relevant for associating the appropriate skill to each food item during actual bite sequencing. We then pass the recognized semantic labels to GroundingDINO~\cite{liu2023grounding}, an open-vocabulary VLM, for bounding box detection. For each bounding box, we use SegmentAnything (SAM)~\cite{kirillov2023segment} to refine these bounding boxes into segmentation masks $\{m^1_t, m^2_t, \hdots, m^D_t\}$ for all $D$ items detected. 

% \begin{lstlisting}
% # Input: Plate image o_t with spaghetti and 3 meatballs, in_context_examples for few-shot recognition/categorization of foods

% labels_t = GPT4V(o_t, in_context_examples)
% # labels_t = [`spaghetti', `meatball',  
% #             `meatball', `meatball']
% categories_t = GPT4V(o_t, in_context_examples)
% # categories_t = [`noodles', `neat/seafood, 
% #             `meat/seafood', `meat/seafood']
% boxes_t = GroundingDINO(o_t, labels_t)
% # bounding boxes
% masks_t = SAM(boxes_t)
% # segmentation masks
% \end{lstlisting}

\smallskip
\noindent \textbf{Skill Library}
The segmented representations of food which we obtained from VLMs provide a useful way to parameterize food manipulation skills, which we split into \emph{acquisition} and \emph{pre-acquisition} skills.


\smallskip
\subsubsection{Acquisition skills} Acquisition skills refer to those that pick up food, such as skewering a food item, twirling a pile of noodles, scooping a soft pile of food, or dipping an item to coat it in sauce. We parameterize them as follows, assuming access to a segmentation mask $m_t$ for the item of interest:
\begin{grayitemize}
    

    \item \underline{\hl{\texttt{skewer}$(x_c, y_c, z_c,\gamma)$}}: We detect the centroid of $m_t$ and deproject this 2D pixel coordinate to a 3D coordinate $(x_c, y_c, z_c)$ representing the center of a food item in the robot's frame of reference. We also estimate the \emph{major-axis} orientation $\theta$ of an item from $m_t$ analytically. Following~\cite{feng2019robot, sundaresan2023learning}, we bring the utensil above the the food item center with $\gamma = 90^{\circ} + \theta$ and execute a swift downward trajectory skewering perpendicular to the main axis of the item. This encourages the tines of the fork to pierce the item. If the tines align parallel to the item's major axis, they may run along its longer length and miss the shorter breadth due to slight calibration challenges, leading to unsuccessful skewering. 
    \item \underline{\hl{\texttt{twirl}$(x_d, y_d, z_d,\gamma)$}}: We adopt the parameterization from VAPORS~\cite{sundaresan2023learning}, a long-horizon system for noodle acquisition.  Specifically, we twirl noodles by bringing the fork to the sensed \emph{densest} pile $(x_d, y_d, z_d)$  on the plate, estimated via 2D Gaussian filtering on $m_t$, and with $\gamma$ identical to the parameterization for skewering (orthogonal to the major axis of the noodle pile sensed via a pose estimation network from~\cite{sundaresan2023learning}). We actuate the roll joint of the fork to complete two full twirls, wrapping noodles on the fork.
    \item \underline{\hl{\texttt{scoop}$(x_s, y_s, z_s, x_d, y_d, z_d)$}}: The fork starts with tines horizontal to the plate and scoops from the \emph{sparsest} region $(x_s, y_s, z_s)$ to the \emph{densest} region $(x_d, y_d, z_d)$ on the plate. This helps consolidate soft foods while picking up the largest bite. \added{We define the sparsest region 
    as the point on the boundary of the food item mask that is furthest from the \emph{densest} region, with the condition that the line connecting these points is not intersected by other food items, such as fillings.  If all potential lines are intersected by other food items, the \emph{sparsest} region defaults to simply the furthest boundary point.}
    \item \underline{\hl{\texttt{dip}$(x_c, y_c, z_c)$}}: Finally, dipping entails bringing a fork containing a food item into the center $x_c, y_c, z_c$ of a small dish containing sauce. We initially orient the fork with tines horizontal to the plate to avoid the food item slipping off the utensil during dipping.
\end{grayitemize}
Immediately following each of these actions, the robot moves the fork tines in a scooping motion by actuating the utensil's pitch joint. The resulting horizontal fork helps prevent items from slipping off the fork after being picked up.

\subsubsection{Pre-acquisition skills} When the above acquisition skills are not immediately feasible due to occlusion from other items or the anticipated amount of food to be picked up being insufficient, we employ a number of auxiliary strategies which we refer to as \emph{pre-acquisition} skills. 
These actions do not directly pick up food but rearrange or manipulate items to facilitate subsequent acquisition. Grouping noodles into a pile before twirling, pushing a meatball off of a bed of spaghetti before twirling, or cutting banana into a bite-sized piece before eating are all examples of pre-acquisition. We parameterize them as follows:

\begin{grayitemize}
    \item \underline{\hl{\texttt{group}$(x_s, y_s, z_s, x_d, y_d, z_d)$}}: For a pile of food distributed on the plate, we sense the densest $(x_d, y_d, z_d)$ and sparsest $(x_s, y_s, z_s)$ regions via $m_t$ and execute a linear push with the fork from the sparsest to densest point. \deleted{ as in~\cite{sundaresan2023learning}}
    \item \underline{\hl{\texttt{push}$(x^i_c, y^i_c, z^i_c, x^j_s, y^j_s, z^j_s)$}}: For a food item with mask $m^i_t$ obstructing a pile of food (such as noodles or a semisolid) with mask $m^j_t$, we can execute a linear push motion starting at the centroid of the obstructing item, \deleted{to the sparsest point of the bed of food underneath.} \added{to the nearest boundary point of the underlying food bed $m^j_t$.}
    \item \underline{\hl{\texttt{cut}$(x_b, y_b, z_b, \gamma)$}}: To cut a food item, we estimate a point on the object $(x_b, y_b, z_b)$ that would result in a bite-sized portion once cut. In practice, we detect the major axis of $m_t$ and traverse a fixed unit length from the one end of the axis to estimate this. We bring the fork horizontal, with $\gamma$ orthogonal to the major axis as in skewering and twirling, and execute a swift downward trajectory to slice the soft item.
    
\end{grayitemize}

% \smallskip
% \noindent \textbf{Skill Library}
% \todo{priya}{Ignore below... todo}
% \begin{grayitemize}
%     \item \underline{\hl{\texttt{skewer($\texttt{x}, \texttt{y}, \texttt{z}, \gamma$)}}} 
%     \item \underline{\hl{\texttt{twirl($\texttt{x}, \texttt{y}, \texttt{z}, \gamma$)}}}
%     \item \underline{\hl{\texttt{group($\texttt{x}_{\small{\texttt{start}}}, \texttt{y}_{\small{\texttt{start}}}, \texttt{z}_{\small{\texttt{start}}}, \texttt{x}_{\small{\texttt{end}}}, \texttt{y}_{\small{\texttt{end}}}, \texttt{z}_{\small{\texttt{end}}})$}}}: 
%     \item \underline{\hl{\texttt{push($\texttt{x}_{\small{\texttt{start}}}, \texttt{y}_{\small{\texttt{start}}}, \texttt{z}_{\small{\texttt{start}}}, \texttt{x}_{\small{\texttt{end}}}, \texttt{y}_{\small{\texttt{end}}}, \texttt{z}_{\small{\texttt{end}}})$}}} 
%     \item \underline{\hl{\texttt{scoop($\texttt{x}_{\small{\texttt{start}}}, \texttt{y}_{\small{\texttt{start}}}, \texttt{z}_{\small{\texttt{start}}}, \texttt{x}_{\small{\texttt{end}}}, \texttt{y}_{\small{\texttt{end}}}, \texttt{z}_{\small{\texttt{end}}})$}}}
%     \item \underline{\hl{\texttt{dip($\texttt{x}, \texttt{y}, \texttt{z}, \gamma$)}}:} 
%     \item \underline{\hl{\texttt{cut($\texttt{x}, \texttt{y}, \texttt{z}, \gamma$)}}:} 
% \end{grayitemize}

$\mathcal{L} = \{\texttt{skewer}, \texttt{twirl}, \texttt{scoop}, \texttt{dip}, \texttt{group}, \texttt{push}, \texttt{cut}\}$ forms the library of vision-parameterized skills at the core of \flair. 

We provide further details on the vision-based parameterizations for each of these skills in the Appendix.

\smallskip
\noindent \textbf{Task Planning for Acquisition.} We plan a sequence of bites that both satisfies the preference of the user, and is efficient for the robot to acquire. The latter consideration requires reasoning over the sequence of pre-acquisition and acquisition skills needed to pick up an item, for which we introduce a hierarchical task planner $\mathcal{T}$. The only parameters the task planner relies on are the density, entropy, and bite size thresholds. Even these are shared across categories of foods like noodles, semisolids, and cuttable items, rendering the approach general enough to handle many different foods.

The task planner takes as input a particular food item category $c^i_t$ along with the detected segmentation mask $m^i_t$ and outputs a sequence of skills to acquire the item. The skill library in this work addresses the following categories of food items: $\{\texttt{`meat/seafood'}, \texttt{`fruit'}, \texttt{`vegetable'}, \texttt{`sauce'},\\ \texttt{`noodles'},\texttt{`semisolid'},  \texttt{`cuttable'} \}$. 

For most categories, acquisition tends to be immediately possible. Food items such as a bite of $\{\texttt{`meat/seafood'},$ $ \texttt{`fruit'}, \texttt{`vegetable'}\}$ tend to be isolated on a plate and immediately acquirable. Thus, we plan the following acquisition skills, where $p^i_t$ denotes the parameters of the skill to manipulate the $i$-th food item, sensed from $m^i_t$ and $o_t$:

\begin{grayitemize}
    \item $\mathcal{T}(c^i_t, m^i_t) = \{\texttt{skewer}(p^i_t)\}$ for \\ $c^i_t \in \{\texttt{`meat/seafood'}, \texttt{`fruit'}, \texttt{`vegetable'}\}$ 
    \item $\mathcal{T}(\texttt{`sauce'}, m^i_t) = \{\texttt{dip}(p^i_t)\}$
\end{grayitemize}

 Food items that are instead in the $\texttt{`noodles'}$, $\texttt{`semisolid'}$, or $\texttt{`cuttable'}$ category require more nuanced reasoning about pre-acquisition depending on the distribution of the food on the plate, and whether other food items are intermixed, on top, or to the side. 
 We critically observe that the segmentation mask $m^i_t$ obtained from the VLM provides a useful prior over the spread of food on the plate, which can guide action selection. 
 We apply a Gaussian smoothing kernel over $m^i_t$ which has the effect of producing a normalized density heatmap of the food,
 % \priya{make a fig for dis}
 and use simple pre-conditions to determine a sequence of skills to pick up a bite of noodles or a semisolid.
Specifically, we measure the maximum \emph{density} and the 2D \emph{entropy} of the heatmap and plan actions as follows.

If the density exceeds a pre-defined threshold $\texttt{DENSITY\_THRESH}$, this indicates the presence of a large pile of food that can be immediately acquired:
\begin{grayitemize}
    \item  $\mathcal{T}(\texttt{`noodles'}, m^i_t) = \{\texttt{twirl}(p^i_t)\}$
    \item $\mathcal{T}(\texttt{`semisolid'}, m^i_t) = \{\texttt{scoop}(p^i_t)\}$.
\end{grayitemize}

Otherwise, when the entropy exceeds a pre-defined threshold $\texttt{ENTROPY\_THRESH}$, indicating that items are spread out on the plate, grouping is necessary before acquiring. We can directly execute unobstructed grouping actions. However, if another item mask $m^j_t$, such as a meatball, intersects with a planned grouping action for spaghetti (Fig. \ref{fig:front}), we instead push the topping aside, group the food, and then acquire.

% Otherwise, when the entropy exceeds a pre-defined threshold $\texttt{ENTROPY\_THRESH}$, this indicates that the items are spread out over the plate and grouping is necessary before acquiring. We can simply execute unobstructed grouping actions. If instead another item mask $m^j_t$ intersects with a planned grouping action, such as a meatball blocking grouping of spaghetti (i.e. Fig. \ref{fig:front}), we instead push the topping aside, group the food, and then acquire.
\begin{grayitemize}
    \item  $\mathcal{T}(\texttt{`noodles'}, m^i_t) = \{\texttt{group}(p^i_{t,\texttt{group}}), \texttt{twirl}(p^i_{t,\texttt{twirl}})\}$ if grouping is unobstructed.
\end{grayitemize}
\begin{grayitemize}
    \item $\mathcal{T}(\texttt{`noodles'}, m^i_t) = \{\texttt{push}(p^i_{t,\texttt{push}}), \texttt{group}(p^i_{t,\texttt{group}}), \\ \texttt{twirl}(p^i_{t,\texttt{twirl}})\}$ if the robot must push aside a topping before twirling.
    \item $\mathcal{T}(\texttt{`semisolid'}, m^i_t) = \{\texttt{push}(p^i_{t,\texttt{push}}), \texttt{scoop}(p^i_{t,\texttt{scoop}})\}$ if the robot must push aside a topping before scooping.
\end{grayitemize}

Finally, for $\texttt{cuttable}$ items like cake, we use a max major-axis length threshold to determine if $m^i_t$ is bite-sized or not, and either cut and then skewer, or skewer immediately:
\begin{grayitemize}
    \item $\mathcal{T}(\texttt{`cuttable'}, m^i_t) = \{\texttt{cut}(p^i_{t,\texttt{cut}}), \texttt{skewer}(p^i_{t,\texttt{skewer}})\}$, if the length of major axis of $m^i_t$ exceeds $\texttt{BITE\_SIZE}$
    \item $\mathcal{T}(\texttt{`cuttable'}, m^i_t) = \{\texttt{skewer}(p^i_t)\}$, otherwise
\end{grayitemize}

\subsection{Bite Sequencing via Foundation Models}
We introduce a unified framework for planning and executing bite sequences that are efficient and adhere to user preferences. With access to a library of skills $\mathcal{L}$, task planner $\mathcal{T}$, and user preference $\ell_{pref}$, we show how the commonsense-reasoning capabilities of LLMs enable them to act as few-shot planners for bite sequencing, inherently balancing preference and efficiency.

We prompt an LLM, in our case GPT-4V with relevant context about the meal. This includes the semantic food item labels $l_t$ and the user's preference $\ell_{pref}$. We augment this context with: (i) a \emph{history} of bites taken so far, (ii) an estimate of the \emph{portions} of each food type remaining, and (iii) the \emph{per-item efficiencies} which correspond to the number of actions required to pick up a food item (i.e. $|\mathcal{T}(c^i_t, m^i_t)|$). A higher number indicates a less efficient bite option since more pre-acquisition skills are required to pick up the item. To estimate quantities, we simply count the number of instances detected of the food item present if the item category is $[\texttt{`fruit'}, \texttt{`meat/seafood'}, \texttt{`vegetable'}]$. Otherwise, we use $\lceil m_t/\texttt{BITE\_SIZE}\rceil$ as a proxy for quantifying the number of bites present, which approximates the number of bite portions in a mask based on a pre-defined portion size. This is necessary for food items where the ground truth quantity is not countable, such as for $\texttt{`noodles'}$ or $\texttt{`semisolid'}$ items.

Below, we show an example input prompt in gray with the immediate next bite planned by asking the LLM to perform completion. We abridge the prompt here for brevity, but include our full prompting strategy in Appendix.

% Include TeX code inside a box
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, boxrule=0.1pt, sharp corners, fontupper=\small, left=0pt,]
\begin{verbatim}
Items remaining: ["fettuccine", "chicken", "broccoli"]
Preference: "Alternating bites of each"
History: ["chicken"]
Portions remaining: [5, 1, 2]
Effiencies: [3, 1, 1]
---
Decide what bite to feed me next.
Format your response as follows:
Strategy: Sentence describing your high-level strategy
Next bite: Phrase describing the next bite you will feed
Next bite as list: ['item'] # Or ['item', 'dip'] or []
---
Output your response here.
\end{verbatim}
\end{tcolorbox}
\begin{tcolorbox}[colback=orange!10, colframe=gray!40, boxrule=00pt, sharp corners, fontupper=\small, left=0pt,]
\begin{verbatim}
Strategy: Given that you want to alternate amongst the
three types of items present, and you just ate chicken,
I will feed you either fettucine or broccoli.
Even though broccoli is a more efficient option, with only
1 action required, I will feed you fettuccine since 
there are more portions of it.
Next bite: Feed fettuccine.
Next bite as list: ['fettuccine']
\end{verbatim}
\end{tcolorbox}

By reasoning about the provided context in a chain-of-thought style, the LLM generates a subsequent bite. Importantly, there are no explicit tradeoffs between efficiency, portion size, or preference which we embed into the prompt, allowing the LLM to reason about the most sensible strategy based on the intensity of the user's preference and available plate context. Given a next bite, in this case $\texttt{`fettuccine'}$, we then plan the appropriate skill sequence via $\mathcal{T}(\texttt{`noodles'}, m^{\texttt{`fettuccine'}}_t$) and execute it via $\mathcal{L}$.
% \flair~ performs long-horizon bite acquisition in an MPC-style approach where after each acquired bite, we update last bite in the history $h_t$ and re-prompt the LLM to obtain a next bite.

\subsection{Integration of Acquisition and Transfer}
The self-contained nature of our \textit{bite acquisition} framework presented in \cref{sec:bite_acq} allows for straightforward integration with \emph{bite transfer} frameworks, and is agnostic to the exact approach used. We demonstrate this easy combination with two existing methods: (i) an outside-mouth bite transfer method~\cite{gallenberger2019transfer} that features visual servoing capabilities, and (ii) a recent method for inside-mouth transfer~\cite{jenamani2024bitetransfer} that leverages robust mouth tracking and physical interaction-aware control.

A significant challenge in this integration is ensuring that food, particularly semi-solid items such as mashed potatoes or noodle-like items such as spaghetti, does not spill while it moves from above the plate to the pre-transfer pose infront of the mouth. Prior works with non-actuated utensils \cite{park2020active} use an MPC-based approach to generate robot trajectories that constrain the orientation of the utensil to remain upright. However, these methods often require complex tuning and can be prone to getting trapped in local minima. Our feeding utensil enables us to uniquely circumvent this challenge. We leverage its roll ($\gamma$) and pitch ($\beta$) degrees of freedom, distinct from the robot's own degrees of freedom, to consistently keep the fork's tines horizontal regardless of the robot's motion. We continuously monitor the robot's end-effector pose at 10 Hz and adjust the feeding utensil's joints accordingly, ensuring a smooth and spill-free transfer of food to the user's mouth.

% \flair's modular composition of acquisition with transfer allows for feeding a wide range of complete meals with a efficient bite sequence that adheres to user preferences. 

\input{figures/plates}

==> inputs/problem_statement.tex <==
\section{Problem Statement}
